Multi-modal Attribute Prompting for Vision-Language Models

Pre-trained Vision-Language Models (VLMs), like CLIP, exhibit strong generalization ability to downstream tasks but struggle in few-shot scenarios. Existing prompting techniques primarily focus on global text and image representations, yet overlooking multi-modal attribute characteristics. This limitation hinders the model's ability to perceive fine-grained visual details and restricts its generalization ability to a broader range of unseen classes. To address this issue, we propose a Multi-modal Attribute Prompting method (MAP) by jointly exploring textual attribute prompting, visual attribute prompting, and attribute-level alignment. The proposed MAP enjoys several merits. First, we introduce learnable visual attribute prompts enhanced by textual attribute semantics to adaptively capture visual attributes for images from unknown categories, boosting fine-grained visual perception capabilities for CLIP. Second, the proposed attribute-level alignment complements the global alignment to enhance the robustness of cross-modal alignment for open-vocabulary objects. To our knowledge, this is the first work to establish cross-modal attribute-level alignment for CLIP-based few-shot adaptation. Extensive experimental results on 11 datasets demonstrate that our method performs favorably against state-of-the-art approaches.

==> sec/0_abstract.tex <==
\begin{abstract}
Large pre-trained Vision-Language Models (VLMs), like CLIP, exhibit strong generalization ability to downstream tasks but struggle in few-shot scenarios.
Existing prompting techniques primarily focus on global text and image representations, yet overlooking multi-modal attribute characteristics. This limitation hinders the model's ability to perceive fine-grained visual details and restricts its generalization ability to a broader range of unseen classes. To address this issue, we propose a Multi-modal Attribute Prompting method (MAP) by jointly exploring textual attribute prompting, visual attribute prompting, and attribute-level alignment. The proposed MAP enjoys several merits. First, we introduce learnable visual attribute prompts enhanced by textual attribute semantics to adaptively capture visual attributes for images from unknown categories, boosting fine-grained visual perception capabilities for CLIP. Second, the proposed attribute-level alignment complements the global alignment to enhance the robustness of cross-modal alignment for open-vocabulary objects. To our knowledge, this is the first work to establish cross-modal attribute-level alignment for CLIP-based few-shot adaptation. Extensive experimental results on 11 datasets demonstrate that our method performs favorably against state-of-the-art approaches.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

 \begin{figure}[t]
  \centering
  \scalebox{0.8}{  \includegraphics[width=0.99\linewidth]{images/for_printv.pdf}}
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
 
\vspace{-0.3cm}
   \caption{(a) Conventional prompting methods use hand-crafted or learnable context in combination with the class name to construct the text prompt. 
   % The image classification result depends on the matching score between the global image feature and the encoded text prompt. 
   (b) Recent methods introduce attribute descriptions to create text attribute prompts containing more semantic content. (c) Our method jointly explores multi-modal attributes and attribute-level alignment, enhancing fine-grained visual perception and achieving attribute-level alignment between images and text categories. }
   \vspace{-0.3cm}
   \label{fig:contra}
\end{figure}
Large-scale pre-trained Vision-Language Models (VLMs), such as CLIP~\cite{CLIP} and  ALIGN~\cite{ALIGN}, have demonstrated promising generalization power and transferability on a wide range of downstream tasks, including image
classification~\cite{CLIP}, object detection~\cite{f-vlm,vlm-adapt2,vlm-adapt3}
and 3D understanding~\cite{3dscene,3d-2,3d-3}.
%
Through contrastive training on a large-scale dataset of image-text pairs, CLIP achieves a global alignment between images and textual descriptions by learning a joint embedding space. The robust cross-modal alignment empowers the CLIP model with the open-vocabulary visual recognition capability. 
In CLIP, class-specific weights for open vocabulary classification can be constructed by plugging the \textbf{class name} in a predefined prompt template like `A photo of a [CLASS].'
Despite its impressive generalization capability, it remains challenging to adapt CLIP to downstream tasks in few-shot scenarios.  The extensive size of the CLIP model and the limited training data available make it unfeasible to fine-tune the complete model for use in downstream few-shot tasks.

To enhance the few-shot adaptation capability of CLIP, prompting techniques~\cite{CoOp,cocoop,dapt,PromptSRC,ProDa,rpo,Maple}, such as CoOp~\cite{CoOp} and CoCoOp~\cite{cocoop} have been proposed. 
 These techniques replace hard template context with learnable context in combination with the class name to construct the text prompt. The classification result can be obtained by calculating the similarity between the global image feature and the encoded text prompt. However, as shown in Figure \ref{fig:contra} (a), these prompting methods rely solely on class names and may struggle to fully encapsulate categorical semantics when new unseen classes emerge, causing an issue of `lexical weak tie' where the class name has a tenuous link with its literal semantics. Consider `Rocky Road' as an example, which textually resembles `rock' and `road' but refers to a dessert in reality. When introduced as a new class, the classification weight generated by the model may diverge from its true semantics, potentially causing misclassification. To address this issue, recent works~\cite{Multi-des,classification_via_des,gpt_enhance_clip}, as shown in Figure \ref{fig:contra} (b), introduce \textbf{textual attribute} descriptions obtained from Large Language Models~\cite{gpt3,gpt4,llmsurvey}. These textual attribute descriptions are appended to the class name to construct text attribute prompts enriched with more semantics. The final classification result is determined by matching scores between the global image feature and the outputs of text attribute prompts across categories.



\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \scalebox{0.6}{   \includegraphics[width=0.99\linewidth]{images/motivation.pdf}}

\vspace{-0.3cm}
   \caption{(a) Moon Orchid and (b) Japanese Anemone exhibit strikingly similar overall appearances.  Visual attributes play a crucial role in distinguishing between them, such as the central yellow stamens of Japanese Anemone.}
   \vspace{-0.7cm}
   \label{fig:visual_attribute}
\end{figure} 


Despite the performance improvements demonstrated by prior methods, two crucial aspects have been overlooked. \textbf{(1) Visual Attribute Modeling.} Previous methods rely on a single global image feature for classification (see Figure \ref{fig:contra} (a) and (b)). However, global image features may fall short in capturing fine-grained visual attribute information crucial for distinguishing visually similar classes in few-shot scenarios. As shown in Figure~\ref{fig:visual_attribute}, the Moon Orchid and Japanese Anemone exhibit quite similar overall appearances, making it challenging to differentiate between them relying solely on global features. However, distinguishing them becomes much easier by relying on their distinct leaf shapes and reproductive structures.  \textbf{(2) Attribute-Level Alignment.} 
The open-vocabulary visual recognition ability of the CLIP model stems from its global alignment between global image features and textual descriptions. However, when adapted to unseen tasks, the global alignment may lack robustness against disruptions from complex image backgrounds and irrelevant image details, hampering the image recognition ability. While previous methods have attempted to model class-specific textual attributes, as depicted in Figure \ref{fig:contra} (b), they still focus on alignment with the global image features and fall short in addressing disruptions present in images. To address this issue, in addition to the global alignment, establishing \textbf{attribute-level alignment} is imperative, \textit{i.e}., alignment between fine-grained visual and textual attribute features (see Figure \ref{fig:contra} (c)). This alignment empowers the model to selectively emphasize the distinctive visual attribute features described in the textual attributes, thereby enhancing the ability to handle disruptions in images.
% Therefore, the CLIP model can handle disruptions in images better.
% and interferences.
% Consequently, the CLIP model becomes better equipped to adapt to complex contexts and disruptions.
% Therefore, it is imperative to construct \textbf{attribute-level alignment}， ， which means 
% to enhance robustness and facilitate
% selective focus on discriminative visual features described in the textual attributes. 

% Therefore, it is imperative to construct \textbf{attribute-level alignment} between fine-grained visual and text attribute features to enhance robustness and facilitate
% selective focus on discriminative visual features described in the textual attributes. 
% 文本属性和全局特征对齐
%CLIP全局对齐的缺点，文本属性仍然是在和全局对齐
%between visual attribute and textual attribute features, 
 

 
%preliminary->initial
 
Inspired by the above insights, we propose  \textbf{Multi-modal Attribute Prompting} (MAP) by jointly exploring textual attribute prompting, visual attribute prompting, and attribute-level alignment to enhance the adaptability of CLIP in downstream few-shot tasks.  For \textbf{textual attribute prompting}, we generate class-specific textual descriptions using a pre-trained large language model. Subsequently, these textual descriptions are utilized to create multiple textual attribute prompts, each encompassing context words, the class name, and an attribute description. It's challenging to directly capture appropriate discriminative visual attributes in an unknown test image without prior information. Hence, for \textbf{visual attribute prompting}, first, we use learnable initial visual attribute prompts to aggregate regional features by interacting with image tokens. Then, we utilize the specially designed \textbf{Adaptive Visual Attribute Enhancement} (AVAE) module, in which the initial visual attribute prompts are enhanced by adaptively selected textual attribute prompts. Through interaction with both image tokens and textual attribute prompts, visual attribute prompts can adaptively capture visual attribute features in an unseen image. Finally, we reformulate the \textbf{attribute-level alignment} between visual attribute prompts and textual attribute prompts as an Optimal Transport problem~\cite{OT} and use the Sinkhorn algorithm~\cite{sinkhorn} to solve it. The ultimate classification result is determined by both the global matching score and the attribute-level matching score. This integration of additional attribute alignment, alongside global alignment, achieves multi-level robust alignment between images and text categories.

% Building upon global alignment, the introduction of additional attribute alignment achieves multi-level robust alignment between images and text categories.


% The combination of additional attribute-level alignment and global alignment achieves multi-level robust alignment between images and text categories.
%不仅需要全局对齐
% The additional attribute-level alignment is combined with the global alignment to achieve multi-level robust alignment between images and text categories.

% We introduce learnable \textbf{visual attribute prompts} within the image encoder to model visual attribute features.  To address this, We design an \textbf{Adaptive Visual Attribute Enhancement} (AVAE) module for progressive refinement of visual attribute prompts. AVAE is placed in the middle layer of the vision encoder and takes initial visual attribute prompts from shallow encoder layers as input. These initial prompts encode regional features of the current image. With these visual regional features, AVAE adaptively enhances the visual attribute prompts using relevant text attribute features.  These enhanced visual attribute prompts are then used to extract visual attribute features in the remaining vision encoder layers. 
% Finally, as in Figure \ref{fig:contra} (c), we reformulate the \textbf{attribute-level alignment} between visual attribute features and textual attribute prompts as an Optimal Transport problem~\cite{OT} and use the Sinkhorn algorithm~\cite{sinkhorn} to solve it. 
% Through the joint exploration of multimodal attributes and attribute-level alignment, MAP enhances fine-grained visual perception ability and achieves more robust alignment between images and corresponding categories in the latent space.
% jointly models visual and text attributes, enhancing the alignment between visual and text features and improving the model's fine-grained visual perception capability.

 

% The MAMN framework presents an innovative approach to jointly capture and leverage both visual and textual attribute information, ultimately enhancing the understanding and classification of visual content.

% Optimal Transport (OT) is then employed to align the visual attribute features and textual attribute features produced by the encoders, considering attribute features as two discrete distributions.






The contributions of our method could be summarized in three-fold: (1) We propose \textbf{Multi-modal Attribute Prompting}, which jointly explores textual attribute prompting, visual attribute prompting, and attribute-level alignment between images and text categories.
(2) We enhance fine-grained visual perception ability by modeling visual attribute features with visual attribute prompts. Moreover, we introduce attribute-level alignment, complementing global alignment, to achieve multi-level robust alignment between images and text categories. To our knowledge, this is the first work to model visual attributes and establish attribute-level alignment between images and text categories for adapting the pre-trained CLIP model to downstream few-shot tasks.
% To the best of our knowledge, this is the first work to jointly model multimodal attributes to enhance the adaptability of VLMs in downstream tasks.  
% (2) Directly modeling discriminative visual attribute features is challenging; we design an \textbf{Adaptive Visual Attribute Enhancement} module to progressively refine visual attribute prompts. 
(3) Extensive experimental results on 11 benchmark datasets demonstrate that our method performs favorably against state-of-the-art approaches.


 

==> sec/Limitation.tex <==
\section{Limitation and Future Work}
We use text attributes directly from GPT without manual filtering. Text attributes may contain noise that may hinder accurate classification, such as attributes with high uncertainty, like colors of toad lilies (white, purple, pink, or yellow). On Flowers102~\cite{flowers}, we manually filter improper attributes, resulting in an improvement of 0.37\% in HM. Filtering improper ones has the potential to improve results. We'll design an automatic filter plan in the future.

==> sec/conclusion.tex <==
\section{Conclusion}
% In this paper, we propose Multi-modal Attribute Prompting to adapt pre-trained Vision-Language models for downstream few-shot tasks. Our method involves modeling visual attributes to enhance the visual fine-grained perception ability. We establish attribute-level alignment, complementing the global alignment for multi-level robust alignment between images and text categories. Experiments demonstrate the effectiveness.
In this paper, we propose a Multi-modal Attribute Prompting method to adapt pre-trained Vision-Language models for downstream few-shot tasks. Our method involves modeling visual attributes to enhance the visual fine-grained perception ability. We establish attribute-level alignment, complementing the global alignment to achieve multi-level robust alignment between images and text categories. Extensive experimental results demonstrate the effectiveness.

==> sec/flops.tex <==
\section{Analysis of Complexity}
Table \ref{tab:Complexity} summarizes the complexity analysis of MAP and previous 
methods. Compared with MaPLe, MAP is more parameter-efficient (0.74M vs 3.56M). 
The GFLOPs of MAP Attribute higher, but considering the performance 
improvement, it is acceptable.
\begin{table}
    
     \caption{Complexity results.}
     \vspace{-0.4cm}
      \centering
        \footnotesize
    \scalebox{1}{  
    \begin{tabular}{l | l l l }
          \toprule
               & CoCoOp  & MaPLe  & MAP   \\ \hline
           params & 0.04M & 3.56M & 0.74M  \\ 
          GFLOPs & 83.83 & 55.23 & 84.80  \\ 
            % CLIP+CoOp+VPT & 83.24 & 70.04 & 75.51  \\ 
            % CLIP+TAP & 83.09 & 74.22 & 78.09  \\ 
            % CLIP+TAP+VPT & 83.48 & 75.94 & 79.3  \\ 
            test time & 56.70s & 9.58s & 9.79s  \\
     
          \bottomrule
        \end{tabular}
        }
     \vspace{-0.4cm}
      \label{tab:Complexity}
    \end{table}

==> sec/method.tex <==
\section{Method}
\label{sec:method}
In this section, we first provide a concise overview of CLIP~\cite{CLIP}. Then, we present a comprehensive introduction to our proposed multi-modal attribute prompting, as illustrated in Figure \ref{fig:method}, including textual attribute prompting, visual attribute prompting, and attribute-level alignment. The main symbols and instructions are shown in Table~\ref{tab:symbol-table}
% (1) Class-specific descriptions obtained from the large language model are used to \textbf{textual attribute prompts}, enriching semantic content in prompts. (2) \textbf{Visual attribute prompts} are introduced to capture visual attributes. The \textbf{Adaptive Visual Attribute Enhancement} module can enhance visual attribute prompts with textual attribute prompts. (3) The \textbf{attribute-level alignment} is reformulated as an optimal transport problem. (4) The final classification is based on the combination of attribute-level alignment and global alignment.
 












%-------------------------------------------------------------------------
\subsection{Review of CLIP}

The Contrastive Language-Image Pre-training (CLIP) model~\cite{CLIP} is a well-known vision-language model trained on large-scale image-text pairs. CLIP consists of two primary components: an image encoder $\phi(\cdot)$ for converting input images into visual embeddings and a text encoder $\theta(\cdot)$ for encoding textual information. During pre-training, CLIP trains encoders using a contrastive loss objective~\cite{contra}, with the purpose of achieving a global alignment between images and textual descriptions. The CLIP model can be easily applied to downstream tasks.
  
Given a set $\mathcal{V}$ of $\mathcal{C}$ class names, the text prompts $\{{t}_i \}_{i=1}^C$ are formulated as manually designed templates, such as `A photo of a [CLASS].' The classification vectors $\{w_i\}_{i=1}^C $ are derived by passing text prompts $\left\{{t}_i\right\}_{i=1}^C$ to the text encoder: $w_i=\theta(t_i)$. Given an image $x$ and its label $y$, the global image feature $f$ is extracted by the image encoder: $f=\phi(x)$. The classification probability is formulated as
\begin{equation}
  P(y=i|{x})=\frac{\exp \left(\cos \left({w}_i, {f}\right) / \tau\right)}{\sum_{j=1}^C \exp \left(\cos \left({w}_j, {f}\right) / \tau\right)},
  \label{eq:clip_p}
\end{equation}
where $\tau$  is a temperature parameter and $\cos (\cdot,\cdot)$  denotes the cosine similarity.


% \subsection{Review of CoOp}

% Hand-crafted prompt templates for generating textual embeddings demand domain-specific expertise and may yield sub-optimal results. CoOp proposes the soft prompt learning approach. Specifically, the prompt for the $i$-th class given to the text encoder $\theta(\cdot)$ is designed with the following form:
% \begin{equation}
%  \mathbf{p}_i=\left\{\boldsymbol{v}_1, \boldsymbol{v}_2, \ldots, \boldsymbol{v}_M, \boldsymbol{c}_i\right\}
%   \label{eq:p_text}
% \end{equation}
% where $c_i$ is the word embedding for the class name, ${v}_1, \boldsymbol{v}_2, \ldots, \boldsymbol{v}_M$ are learnable vectorss,and $M$ is a hyperparameter specifying the number of context tokens. The prediction probability over the class labels of image x is computed as follows:
% \begin{equation}
%  P(y=i \mid \mathbf{x})=\frac{\exp \left(\cos \left(\theta\left(\mathbf{p}_i\right), \mathbf{f}\right) / \tau\right)}{\sum_{j=1}^C \exp \left(\cos \left(\theta\left(\mathbf{p}_j\right), \mathbf{f}\right) / \tau\right)}
%   \label{eq:p_text_p}
% \end{equation}
% The learnable context vectors are optimized by minimizing the cross-entropy loss: 




\begin{figure*}[t]
  \centering
  % \begin{subfigure}{0.68\linewidth}
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
       \includegraphics[width=0.99\linewidth, ]{images/main.pdf}
       % height=83mm
    % \caption{An example of a subfigure.}
    % \label{fig:short-a}
  % \end{subfigure}
  % \hfill
  \vspace{-0.3cm}
  \caption{The architecture of our method: \textbf{MAP} leverages textual attribute descriptions to construct textual attribute prompts and incorporates learnable visual attribute prompts for capturing visual attributes. In the \textbf{Adaptive Visual Attribute Enhancement} module, initial visual attribute prompts are enhanced by textual attribute prompts via the attribute-aware cross-attention layer. The \textbf{Multi-modal Attribute Alignment} module calculates the similarity score between visual attributes and textual attributes with the optimal transport.}
  \label{fig:method}
\end{figure*}
\vspace{-1.4cm}

\subsection{Textual Attribute Prompting}
To address the potential `lexical weak tie' issue of relying solely on class names for text prompt construction, we create multiple textual attribute prompts for each class, which helps enrich the semantic content in text prompts.




\textbf{Attribute Descriptions.} Consistent with previous methods~\cite{gpt_enhance_clip,classification_via_des,Multi-des}, we obtain category attribute descriptions by querying a Large Language Model (LLM) using a predefined question template: `What are useful visual features for distinguishing a [CLASS] in an image?' In response, the LLM provides discriminative attribute descriptions for the queried class. We select  $N$ descriptions for each class from the query results.


% $A_k=\{a_{k}^1, a_{k}^2, a_{k}^3, a_{k}^4,...\}$ specific to the $k$-th class.

% Given our collection of $N$ LLM-generated attribute descriptions for each of the $C$ classes, where $t_{n,k}$ represents the $n$-th attribute description for the $k$-th class, 
\textbf{Textual Attribute Prompt Construction.} We formulate $N$ textual attribute prompts for each class by combining attribute description sentences with a standardized prompt template. For instance, for the $k$-th class, with the template `A photo of a [CLASS]' we construct a textual attribute prompt: $p_k^n$=\{A photo of a class ($k$), $t_{n,k}$\}, where class ($k$) denotes the class name corresponding to the $k$-th class, and $t_{n,k}$ denotes the $n$-th attribute description for the $k$-th class. To enhance the adaptability of textual attribute prompts, we replace the hand-crafted context, \textit{i.e}., `A photo of a' with several learnable context vectors. 
% Finally, we construct $N$ textual attribute prompts {for each class}:
% \begin{equation}
%   P_k=\{ p_n^k|_{n=1}^N\},
%   \label{eq:p_k}
% \end{equation}
% \textcolor{blue}{where $P_k$ denotes textual attribute prompts of the $k$-class}. 
By feeding the textual attribute prompts into the text encoder $\theta$, we can obtain encoded textual attribute prompts:
\begin{equation}
 \boldsymbol{G}_k=\{{g}_k^n|_{n=1} ^N\}, g_k^n=\theta(p_n^k),
  \label{eq:G_k}
\end{equation}
where $\boldsymbol{G}_k$ is the textual attribute prompt set for the $k$-class.

\subsection{Visual Attribute Prompting}
% Unlike previous approaches~\cite{CoOp,cocoop,gpt_enhance_clip} that depend solely on the global image feature for classification, 
To improve fine-grained visual perception, we model visual attributes with visual attribute prompts. However, it is challenging to directly learn discriminative visual attributes for an unknown image without prior information. Therefore, we design an adaptive visual attribute enhancement module to adaptively establish visual attribute prompts under the guidance of textual attribute information.

\textbf{Learnable Visual Attribute Prompts.} We model visual attributes by introducing $M$ visual attribute prompts $U=\{ u_i\}_{i=1}^M$, where each attribute prompt $u_i$ is a randomly initialized learnable vector with the dimension of $d_v$. $\{ u_i\}_{i=1}^M$ are inserted into the first Vision Transformer (ViT) layer and are then propagated into deeper layers.
%s that consist of Self-Attention and Feed-Forward sub-layers~\cite{vit}. 
%the first Vision Transformer (ViT) layer $\l_1$. 
%Each transformer layer $l_j$ consists of Self-Attention and Feed-Forward Networks~\cite{vit}. 
%We denote the collection of attribute prompts $\{ u_i\}_{i=1}^M$ as $U_0$. 
For the $j$-th ViT layer $l_j$, visual attribute prompts $U_{j-1}$ output from the ($j$-1)-th ViT layer are concatenated with image tokens $E_{j-1}$ and the learnable classification token $s_{j-1}$ ([CLS]), forming the input sequence of the current layer.
Formally,
%The $j$-th prompted ViT layer $l_j$ is formulated as
\begin{equation}
[s_j,U_j,E_j]=l_j([s_{j-1},U_{j-1},E_{j-1}]), j=1,2,...,L,
  \label{eq:vit}
\end{equation}
where $[\cdot,\cdot]$ indicates the concatenation along the sequence length dimension. In early layers of ViT, the visual attribute prompts progressively aggregate image regional features through interaction with image tokens. 
% \textcolor{red}{The final outputs of ViT include the global image feature $s_L$, visual attribute prompts $U_L=\{ u_i^{(L)}\}_{i=1}^M$.}
% and $E_L$. 
% $s_L$ is the global image feature and $Z_L$ i.e. $\{ u_i^{(L)}\}_{i=1}^M$
% \textcolor{red}{$Z_L=\{ u_i^{(L)}\}_{i=1}^M$ is the set of visual attribute prompts output by ViT.}
% $Z_i \in  \mathbb{R}^{M \times d_v}$ represents the attribute prompts output by the $i$-th transformer layer and 



% $x^{(0)}$ denotes token embeddings to be input to the vision encoder layers, $s$ is the class token of the vision encoder, $E^{(0)}\in\mathbb{R}^{\frac{(H\times W)}{S}\times d_t}$ represents the image patch embeddings, where $H$ and $W$ denote the height and width of the input image, $S$ is the patch size, and $d_v$ represents the dimension of image patch embeddings. $u_i \in \mathbb{R}^{d_v}$ signifies the $i$-th learnable visual attribute prompt, while $M$ denotes the number of learnable prompts.

% The output of the image transformer encoder is  expressed as:
% \begin{equation}
%   x^{(L)}=[{s}^{(L)};E^{(L)};\{ {u_i}^{(L)}\}_{i=1}^M]
%   \label{eq:x_L}
% \end{equation}
% where $L$ is the number of transformer layers.
 


\textbf{Adaptive Visual Attribute Enhancement Module.} AVAE, represented as $\mathbf{\Gamma}$, is designed to dynamically refine visual attribute prompts with textual attribute guidance for arbitrary images from unseen classes. As the category of the test image is unknown, we select possibly related textual attribute prompts from the most similar classes. Specifically, we first compute the similarities between the global image feature, \textit{i.e}., the classification token $s$, and textual category embeddings represented by the mean of textual attribute prompts.
Based on these similarities, we select the most similar $\lambda$ categories as the candidate classes 
and gather their textual attribute prompts as $\boldsymbol{G^{\prime}}=\{g_j|_{j=1}^{\lambda N}\}$. Subsequently, the textual attribute prompts 
 $\boldsymbol{G^{\prime}}$
are employed as the semantic guidance to enhance visual attribute prompts at the $l$-th ViT layer:
\begin{equation}
\{{\Tilde{u}_i}^{(l)}\}_{i=1}^M=\mathbf{\Gamma}( \{{u_i}^{(l)}\}_{i=1}^M,\boldsymbol{G^\prime}),
  \label{eq:gamma}
\end{equation}
where $\mathbf{\Gamma}$ takes the  initial visual attribute prompts $\{ {u_i}^{(l)}\}_{i=1}^M$ generated from 
$l$-th layer as the input, and refine them conditioned on textual attribute prompts   $\boldsymbol{G^\prime}$. 
%By Equation~\eqref{eq:gamma}, $\mathbf{\Gamma}$ generates 
Then the enhanced visual attribute prompt ${\Tilde{u}_i}^{(l)}$ is inserted into the ($l+1$)-th layer for progressive attribute learning.


To better inject the semantic clues of selected textual prompts into visual attribute prompts, 
we design an attribute-aware cross-attention layer in $\mathbf{\Gamma}$. Here, the visual attribute prompt tokens $\{{u_i}^{(l)}\}_{i=1}^M$ function as queries $\boldsymbol{Q}$. Simultaneously, the textual attribute prompt features $\boldsymbol{G^{\prime}}$ of candidate classes are utilized as keys $\boldsymbol{K}$ and values $\boldsymbol{V}$. The enhanced visual attribute prompt $\Tilde{u}_i^{(l)}$ is formulated as 
\begin{gather}
\Tilde{\alpha}_{i j}=\frac{\exp({\alpha_{ij}})}{\sum_{j^\prime=1}^{\lambda N} \exp({\alpha_{ij^\prime}})},
{\alpha}_{i j}=\frac{u_i^{(l)}W_Q\cdot (g_jW_K)^T}{\sqrt{d_K}},\\
\Tilde{u}_i^{(l)}=u_i^{(l)}+\sum_{j=1}^{\lambda N }\Tilde{\alpha}_{i j} (g_jW_V), i=1,2, \cdots, \lambda N,
  \label{eq:u_n}
\end{gather}
where $W_Q$,$W_K$ and $W_V$ are linear projections of the attention layer. {Attention scores} $\Tilde{\alpha}_{i j}$ indicate the correspondence between visual and textual attribute prompts, emphasizing relevant image-specific semantic attribute patterns for enhancing the visual attribute prompts. After the text-guided enhancement, the {refined visual attribute prompts $\{\Tilde{u}_i^{(l)}\}_{i=1}^M$ are propagated into the remaining vision encoder layers and continue to capture visual attributes through interaction with image tokens.}



% In the Vision Transformer's early layers, the attention mechanism enables the interaction of initial visual attribute prompts with image tokens,  facilitating the aggregation of image region features to the visual attribute prompts. 


% where $\tilde{\alpha}_{i j}$ denotes the attention score between the $\mathbf{Q}_i$ and $\mathbf{K}_j$, and $\sqrt{d_K}$ acts as a scaling factor.  To be more specific,  the enhanced visual attribute prompt $u_i^{(l)}$ is computed as a weighted sum over all values using the corresponding attention scores. To retain features aggregated by the visual attribute prompt from shallow layers, $u_i^{(l)}$ is also added to the weighted sum.


\subsection{Attribute-Level Alignment}
% Given an image $x$, we input it into the vision encoder to obtain the class token $s^{(L)}$ as the global image feature $f$ and visual attribute features $\{u_i^{(L)}\}_{i=1}^M$. At the same time, we obtain textual attribute features $\boldsymbol{G_k}=\{g_k^n|_{n=1}^N\}$ for the $k$-th class with the text encoder. For simplicity, we will refer to $\{u_i^{(L)}\}_{i=1}^M$  as  $\boldsymbol{F}=\{f_m|_{m=1}^M\} \in \mathbb{R}^{M \times d^{\prime}}$ in the following text.
To achieve precise alignment between visual attribute prompts $ \{{u_i}^{(L)}\}_{i=1}^M$ and textual attribute prompts $\boldsymbol{G_k}=\{g_k^n|_{n=1}^N\}$, we formulate the attribute-level matching task as an Optimal Transport (OT) problem~\cite{OT}. For simplicity, we refer to $ \{{u_i}^{(L)}\}_{i=1}^M$ as $\boldsymbol{F}=\{f_m|_{m=1}^M\} $ hereafter. OT aims to find the optimal transportation plan with the minimal cost between two discrete distributions $\mu \in \mathbb{R}^M$, $\nu \in \mathbb{R}^N$. The optimal transportation plan $\mathbf{T}^*$ is obtained by minimizing the transportation cost:
\begin{equation}
\begin{gathered}
\mathbf{T}^*=\underset{\mathbf{T} \in \Pi(\mu, \nu)}{\arg \min }\langle\mathbf{T}, \mathbf{C}\rangle, \\
\text { s.t. } \quad \mathbf{T} \mathbf{1}=\mu, \mathbf{T}^T \mathbf{1}=\nu,
\end{gathered}
  \label{eq:ot_cost}
\end{equation}
where $\prod(\mu, \nu)$ is the joint distribution with marginals $\mu$ and $\nu,\langle\cdot, \cdot\rangle$ denotes the cosine similarity, and $\mathbf{C} \in \mathbb{R}^{M \times N}$ represents the cost matrix of transporting $\mu$ to $\nu$. The Problem in Equation ~\eqref{eq:ot_cost} can be efficiently solved by the Sinkhorn algorithm~\cite{sinkhorn}. To apply OT to the multi-modal attribute matching task, we formulate the attribute prompt sets as discrete uniform distributions. The cost matrix $\mathbf{C}$ is defined as the distances between attribute prompts. By solving Equation ~\eqref{eq:ot_cost}, we can obtain $\mathbf{T}^*$ to serve as the alignment matrix, and then define the final similarity score between the visual attribute prompts $\boldsymbol{F}$ and textual attribute prompts $\boldsymbol{G}_k$ as:
\begin{equation}
\psi(\boldsymbol{F},\boldsymbol{G}_k)=\sum_{m=1}^M \sum_{n=1}^N<f_m,g_k^n>\mathbf{T}_{mn}^*,
  \label{eq:sim}
\end{equation}
where $\psi(\cdot,\cdot)$ denotes the similarity function.
 



\subsection{Training Objectives}

Based on the attribute-level alignment, we can classify the image $x$ with fine-grained visual attributes:
\begin{equation}
\begin{gathered}
P_a(y=i| {x})=\frac{\exp( \psi \left(\left(\boldsymbol{F}, \boldsymbol{G}_i\right) / \tau\right))}{\sum_{j=1}^C \exp (\psi (\boldsymbol{F}, \boldsymbol{G}_j / \tau))}.
\end{gathered}
  \label{eq:P_a}
\end{equation}
Furthermore, relying on the global alignment in CLIP, the prediction probability is computed as
\begin{equation}
\begin{gathered}
P_g(y=i| {x})=\frac{\exp( \cos\left(\left(\boldsymbol{f}, \overline{\boldsymbol{g}}_i\right) / \tau\right))}{\sum_{j=1}^C \exp (\cos (\boldsymbol{f}, \overline{\boldsymbol{g}}_j / \tau))},
\end{gathered}
  \label{eq:P_g}
\end{equation}
where $\boldsymbol{f}$ is the global feature of the image $x$, \textit{i.e}., the class token $s_L$, and $\overline{\boldsymbol{g}}_i$ is the textual categorical embedding of the $i$-th class, \textit{i.e}., the mean value of textual prompts in $\boldsymbol{G}_i$. The final prediction probability is 
\begin{equation}
\begin{gathered}
P(y=i| {x})=P_g(y=i| {x})+\beta P_a(y=i|{x}),
\end{gathered}
  \label{eq:P_f}
\end{equation}
which incorporates both global-level prediction scores and additional attribute-level matching scores, achieving multi-level robust alignment between images and categorical texts. Naturally, the classification loss is formulated as:
\begin{equation}
\begin{aligned}
 L_{cls}=-\frac{1}{B}\sum_{i=1}^B logP(y=y_i|x_i),
\end{aligned}
  \label{eq:t_loss}
\end{equation}
where $B$ is the batch of image-text pairs, and $y_i$ denotes the ground-truth of $x_i$.

% To combine the benefits of both global alignment and attribute-level alignment, the final prediction result is
% \begin{equation}
% \begin{gathered}
% P(y=i| \mathbf{x})=P_g(y=i| \mathbf{x})+P_a(y=i| \mathbf{x}).
% \end{gathered}
%   \label{eq:P_f}
% \end{equation}

% \textcolor{red}{Training is performed to minimize the standard classification loss based on the cross-entropy.}



























%  \begin{equation}
% \mathcal{L}=-\sum_{i=1}^C \log P(y=i \mid \mathbf{x})
%   \label{eq:c-n-loss}
% \end{equation}
 
% which aims to transport a collection of visual attribute features with a given image to textual attribute features of a corresponding text class. 

% For the given visual attribute features $\boldsymbol{F}_i \in \mathbb{R}^{M \times d^{\prime}}$ and textual attribute features $\boldsymbol{G}_i \in \mathbb{R}^{N \times d^{\prime}}$, we construct two discrete distributions:
  

% \begin{equation}
% \boldsymbol{\mu}=\sum_{m=1}^M u_m \delta_{\boldsymbol{f}_m}, \quad \boldsymbol{v}=\sum_{n=1}^N v_n \delta_{\boldsymbol{g}_n}
%   \label{eq:distribution}
% \end{equation}
% where $\delta_{\boldsymbol{f}_m}$ is a Dirac function centered at $\boldsymbol{f}_m$, so as to $\delta_{\boldsymbol{g}_n}$, and the weights $\boldsymbol{u}=\left\{u_m\right\}_{m=1}^M \in \Delta_N$ and $\boldsymbol{v}=\left\{v_n\right\}_{n=1}^N \in \Delta_N, \Delta$ denotes the $M$- and $N$-dimensional probability simplex, i.e., $\sum_{m=1}^M u_m=1$, $\sum_{n=1}^N v_n=1$. Finally, the discrete OT distance for one sample is defined as follows:



























% \begin{equation}
%  \begin{aligned}
% & D_{\mathrm{OT}}(\boldsymbol{\mu}, \boldsymbol{v})=\min _{\boldsymbol{T} } \sum_{m=1}^M \sum_{n=1}^N \boldsymbol{T}_{m, n} \cdot \boldsymbol{C}_{m, n} \\
% & \text { s.t. } \quad \boldsymbol{T} \mathbf{1}_n=\boldsymbol{\mu}, \quad \boldsymbol{T} \mathbf{1}_m=\boldsymbol{v},
% \end{aligned}
%   \label{eq:D}
% \end{equation}
% where $\boldsymbol{C} \in \mathbb{R}^{M \times N}$ is the cost matrix, and $\boldsymbol{C}_{m, n}$ is the transportation cost between $\boldsymbol{f}_m$ and $\boldsymbol{g}_n$. $\boldsymbol{T} \in \mathbb{R}^{M \times N}$ is the transport plan that is to be optimized. As directly solving the problem is quite time-consuming, we use the Sinkhorn distance to use entropic constraint for fast optimization


% \begin{equation}
% \begin{aligned}
% P(y=i| \mathbf{x})=&\frac{\exp( \cos\left(\left(\boldsymbol{f}, \overline{\boldsymbol{g}}_i\right) / \tau\right))}{\sum_{j=1}^C \exp (\cos (\boldsymbol{f}, \overline{\boldsymbol{g}}_j / \tau))} +\\
% &\frac{\exp( \psi \left(\left(\boldsymbol{F}, \boldsymbol{G}_i\right) / \tau\right))}{\sum_{j=1}^C \exp (\psi (\boldsymbol{F}, \boldsymbol{G}_j / \tau))},
% \end{aligned}
%   \label{eq:p_f}
% \end{equation}

==> sec/relatework.tex <==
\section{Related work}
\label{sec:relatework}
In this section, we introduce several lines of research in pre-trained vision-language models and prompt learning.
 

%-------------------------------------------------------------------------
\textbf{Pre-trained Vision-Language Models.} 
% Few-shot learning, which aims at learning new concepts with limited training samples, heavily relies on the transferability of pretrained neural networks, since it is infeasible to train a neural network with limited training data from scratch.
% Integrating language supervision with natural images has gained significant attention within the computer vision community.  
In recent years, pre-trained vision-language 
models~\cite{CLIP, ALIGN,flava, lit,Florence} have shown exceptional 
performance in diverse downstream tasks. Among them,  CLIP~\cite{CLIP} stands out as a representative approach. By training its vision and text encoders to map both modalities closely in a shared embedding space, CLIP establishes a comprehensive global alignment between images and their corresponding textual descriptions, enabling open-vocabulary classification tasks. The classification result can be obtained by computing the similarity scores of the global image feature with class names encoded by the text encoder. However, as classification relies solely on the global matching score, the accuracy may be affected by disruptions in images, such as complex backgrounds, especially in few-shot settings. To improve the robustness of cross-modal alignment, we achieve multi-level alignment for CLIP by introducing additional attribute-level alignment between dynamically learned textual and visual attribute features. In this manner, our method enhances the fine-grained perception capability with the pre-trained global knowledge preserved. 

%while keeping the encoders frozen.
% Despite its impressive generalization capability, adapting CLIP to downstream tasks in few-shot scenarios remains challenging. 
% The limited training sample available and the extensive size of the CLIP model make it unfeasible to fine-tune the full model for use in downstream tasks.
% Akin to previous methods~\cite{CoOp,cocoop}, our method focuses on the CLIP model, with the goal of effectively adapting the pre-trained vision-language models to downstream few-shot tasks. 
% jointly learn text and image embeddings with transformer-based encoders. These vision-language models have shown remarkable performance in a variety of downstream classification tasks via prompting. 


% \textcolor{red}{[to be added: Pros and Cons, connections with our method]}
% Few-shot learning aims to learn and adapt to new tasks with limited training samples. It is unfeasible to fine-tune the complete vision-language model. Therefore, prompt learning methods have gained significant attention. These methods involve fine-tuning vision-language models with frozen encoders, allowing for effective adaptation to new tasks.

\textbf{Prompt Learning.} Prompt learning is initially introduced in the field of natural language processing (NLP)~\cite{nlp_p1,nlp_p2_autoprompt,nlp_p3,nlp_p4_tune,nlp_p5_tune,nlp_p6_ppt,nlp_p7gpt}. With language models frozen, prompt learning methods effectively facilitate the adaptation of pre-trained language models to downstream few-shot tasks by involving additional hand-crafted or learnable prompt tokens. Prompt learning has recently been employed to enhance the adaptation of the CLIP model to downstream few-shot tasks, where limited training samples are available. CoOp~\cite{CoOp}  constructs prompts by concatenating learnable continuous vectors and class name tokens. CoCoOp~\cite{cocoop} extends CoOp by further learning a lightweight neural network to generate an input-conditional vector for each image, tackling the poor generalizability to broader unseen classes in CoOp~\cite{CoOp}. ProDA~\cite{ProDa} optimizes a set of prompts by learning the distribution of prompts. Instead of focusing on text-modal prompts, VPT~\cite{vpt} introduces learnable vectors to the Vision Transformer~\cite{vit} to refine image features within the frozen vision encoder. DAPT~\cite{dapt}, RPO~\cite{rpo}, and MaPLe~\cite{Maple} improve the generalization ability of VLMs via multimodal prompting. These methods rely solely on class names for text prompt construction and may struggle to fully encapsulate categorical semantics.

\textbf{Textual Attribute Prompts.}  
To enrich the semantic description for different classes,  recent works~\cite{classification_via_des,gpt_enhance_clip, Multi-des}, instead of relying solely on class names, have shifted towards the utilization of attribute descriptions to construct textual attribute prompts for each class. This shift is facilitated by the development of pre-trained large language models (LLMs) like the GPT family~\cite{gpt3,gpt4}. Attribute descriptions can be easily obtained by
querying the LLM with suitable question templates. However, these methods focus on attributes in text space only, neglecting the modeling of visual attributes, leading to limited visual perception capabilities of the model and misalignment between global visual and local textual features. In contrast, we jointly model visual and textual attribute features and establish attribute-level alignment between images and text categories.

% As relying solely on class names for prompt construction may sometimes fail to fully encapsulate categorical semantics, recent works ~\cite{classification_via_des,gpt_enhance_clip, Multi-des} model textual attribute prompts for each class with attribute descriptions. This method are facilitated by the development of pre-trained large language models (LLMs) such as the GPT family~\cite{gpt3,gpt4}. These models enable the easy acquisition of attribute descriptions by querying the LLM with suitable question templates.
% Thanks to the development of pre-trained large language models （LLMs) like GPT-3, attribute descriptions can be easily obtained by querying the language model with suitable question templates.
% questioning GPT yields descriptors for each class, which are then used to construct semantic-enhanced prompts. 

% DAPT~\cite{dapt} optimizes the distribution of embeddings for both visual and textual modalities for better feature alignment. RPO~\cite{rpo} learns read-only prompts to ensure a more robust and generalizable adaptation.


% \subsection{Semantic-enhanced Prompts}
% Using class names alone to construct prompts may sometimes fail to 


% Using class names alone to construct prompts overlooks the rich contextual information that language itself can provide, resulting in a restricted capacity for expressing semantic information. Thanks to the significant strides made in the development of pre-trained Large Language Models (LLMs), it has become feasible to readily acquire class-specific language information by creating suitable question templates tailored for LLMs. Recent works ~\cite{classification_via_des,gpt_enhance_clip, Multi-des} questioning GPT yields descriptors for each class, which are then used to construct semantic-enhanced prompts. 

==> tabs/ab_flops.tex <==
 \vspace{-0.6cm}
\begin{table}[]
    \begin{minipage}[t]{0.5\linewidth}
    \centering
    \caption{Ablation results.}
    \vspace{-0.4cm}
    \label{tab:compoents}
    \begin{threeparttable}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{2pt}
    \small



    \begin{tabular}{@{\hspace{10pt}}c@{\hspace{10pt}}c@{\hspace{10pt}}c|c }
        \toprule
            Method & Base & Novel & HM  \\ \hline
         Baseline & 82.20 & 72.22 & 76.41  \\ 
        +TAP(LLM) & 82.06 & 73.65 & 77.36  \\ 
          +TAP+VAP (MAP) & 83.66 & 75.76 & 79.36  \\
   
        \bottomrule
      \end{tabular}
    }



    \end{threeparttable}
    \end{minipage}
    \begin{minipage}[t]{0.5\linewidth}
    \centering
    \caption{{Complexity results.}}
    \vspace{-0.4cm}
    \label{tab:flops}
    \begin{threeparttable}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{4pt}
    \small

    \begin{tabular}{@{\hspace{10pt}}c|@{\hspace{10pt}}c@{\hspace{10pt}}cc }
        \toprule
             & CoCoOp  & MaPLe  & MAP   \\ \hline
         params & 0.04M & 3.56M & 0.74M  \\ 
        GFLOPs & 83.83 & 55.23 & 84.80  \\ 
          test time & 56.70s & 9.58s & 9.79s  \\
   
        \bottomrule
      \end{tabular}
    }



    \end{threeparttable}
    \end{minipage}
    \vspace{-0.4cm}
    \end{table}

\vspace{-0.3cm}

==> tabs/cross_dataset_copy.tex <==
\begin{table}[!tb]

    \small \centering
 \setlength{\tabcolsep}{8pt}
  \caption{{ Cross-dataset evaluation.} Prompting methods are trained on ImageNet and evaluated on target datasets. MAP achieves overall favorable performance.} 
  \vspace{-0.4cm}
    \scalebox{0.65}[0.65]{
    \begin{tabular}{l cccccccccccc}
    \toprule
    &  {Source} & \multicolumn{10}{c}{ {Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-12}
     & ImageNet  &  {Cal} &  {Pet} &  {Car} &  {Flo} &  {Foo} &  {Air} &  {SUN} &  {DTD} &  {Eur} &  {UCF}\\
    \midrule 
    CoOp &   {71.51} & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & {{46.39}} & 66.55  \\
    CoCoOp & 71.02 &  \textbf{ 94.43} & {90.14} & 65.32 & {71.88} & 86.06 & 22.94 &   {67.36} & 45.73 & 45.37 & 68.21  \\
    MaPLe & 70.72 & 93.53 &   {{90.49}} & \textbf{65.57} &  \textbf{ {72.23}} &   \textbf{{86.20}} &   {{24.74}} & 67.01 & {46.49} & \textbf{  {{48.06}}} & {68.69} &    \\
    \midrule
MAP & \textbf{71.60} &   {93.93} & \textbf{{90.80}} &   {63.00} & {68.40} & {{86.07}} & \textbf{{24.87}} & \textbf{68.10} &   \textbf{51.87} & {{42.63}} &   \textbf{68.73}  \\  
             \midrule

   
    \end{tabular}
    }
       
    \label{tab:cross-data}
    % \vspace{-2em}
\end{table} 

% \begin{table}[!t]
%     \small \centering
%     \scalebox{0.65}{
%     \begin{tabular}{l c ccccccccccc}
%             \caption{{Cross-dataset benchmark evaluation.} MAP achieves overall favorable performance.}
%     \toprule
%     &   {Source} & \multicolumn{10}{c}{  {Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-13}
%     &  {Img} &  {Cal} &  {Pet} &  {Car} &  {Flo} &  {Foo} &  {Air} &  {SUN} &  {DTD} &  {Eur} &  {UCF}  \\
%     \midrule
%     CoOp &   {71.51} & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & {{46.39}} & 66.55  \\
%     Co-CoOp & 71.02 &  { 94.43} & {90.14} & 65.32 & {71.88} & 86.06 & 22.94 &   {67.36} & 45.73 & 45.37 & 68.21  \\
%     MaPLe & 70.72 & 93.53 &   {{90.49}} & {65.57} &  { {72.23}} &   {{86.20}} &   {{24.74}} & 67.01 & {46.49} & {  {{48.06}}} & {68.69} &    \\
%     \midrule
% MAP & 71.60 &   {93.93} & {{90.80}} &   {63.00} & {68.40} & {{86.07}} & {{24.87}} & 68.10 &   {51.87} & {{42.63}} &   {68.73}  \\    
%  % PromptSRC & 71.27 &   {93.60} & {{90.25}} &   {65.70} & {70.25} & {{86.15}} & {{23.90}} & 67.10 &   {46.87} & {{45.50}} &   {68.75} & {{65.81}} \\
%     \bottomrule
%     \end{tabular}
%     }
    
   
%     \label{tab:xd} %\vspace{-1em}
% \end{table}


 

==> tabs/cross_domain.tex <==
\begin{table}[]
    \begin{minipage}[t]{0.335\linewidth}
    \centering
    \caption{Domain generalization evaluation.}
    \vspace{-0.4cm}
    \label{tab:robustness}
    \begin{threeparttable}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{2pt}
    \small



    \begin{tabular}{c ccccc}
        \toprule
        &  {Source} & \multicolumn{4}{c}{ {Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-6}
         & Img & -V2 & -S & -A & -R \\
        \midrule 
        % CLIP &   {66.73} &  {{60.83}} & 46.15  & 47.77  & 73.96  & {57.18} \\
        CoOp &   {71.51} &  {{64.20}} & 47.99  & 49.71  & 75.21  \\
        CoCoOp & 71.02 & {64.07} & 48.75 & 50.63 & 76.18\\
            MaPLe & 70.72  & {64.07} & \textbf{49.15}  & 50.90 & 76.98 \\
            MAP & \textbf{71.60}  & \textbf{64.47} & 49.07  & \textbf{51.07} & \textbf{77.37}   \\
                 \midrule
    
       
        \end{tabular}
    }



    \end{threeparttable}
    \end{minipage}
    \begin{minipage}[t]{0.665\linewidth}
    \centering
    \caption{{Cross-dataset evaluation. Prompting methods are trained on ImageNet 
    and evaluated on target datasets.}}
    \vspace{-0.4cm}
    \label{tab:cross-data}
    \begin{threeparttable}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{2pt}
    \small


    \begin{tabular}{c cccccccccccc}
        \toprule
        &  {Source} & \multicolumn{10}{c}{ {Target}} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-12}
         & Img  &  {Cal} &  {Pet} &  {Car} &  {Flo} &  {Foo} &  {Air} &  {SUN} &  {DTD} &  {Eur} &  {UCF}\\
        \midrule 
        CoOp &   {71.51} & 93.70 & 89.14 & 64.51 & 68.71 & 85.30 & 18.47 & 64.15 & 41.92 & {{46.39}} & 66.55  \\
        CoCoOp & 71.02 &  \textbf{ 94.43} & {90.14} & 65.32 & {71.88} & 86.06 & 22.94 &   {67.36} & 45.73 & 45.37 & 68.21  \\
        MaPLe & 70.72 & 93.53 &   {{90.49}} & \textbf{65.57} &  \textbf{ {72.23}} &   \textbf{{86.20}} &   {{24.74}} & 67.01 & {46.49} & \textbf{  {{48.06}}} & {68.69} &    \\
       
    MAP & \textbf{71.60} &   {93.93} & \textbf{{90.80}} &   {63.00} & {68.40} & {{86.07}} & \textbf{{24.87}} & \textbf{68.10} &   \textbf{51.87} & {{42.63}} &   \textbf{68.73}  \\  
                 \midrule
    
       
        \end{tabular}
    }



    \end{threeparttable}
    \end{minipage}
    \vspace{-0.4cm}
    \end{table}
